Noise-Compensated, Bias-Corrected Diffusion Weighted Endorectal Magnetic Resonance Imaging via a Stochastically Fully-Connected Joint Conditional Random Field Model

Diffusion weighted magnetic resonance imaging (DW-MR) is a powerful tool in imaging-based prostate cancer screening and detection. Endorectal coils are commonly used in DW-MR imaging to improve the signal-to-noise ratio (SNR) of the acquisition, at the expense of significant intensity inhomogeneities (bias field) that worsens as we move away from the endorectal coil. The presence of bias field can have a significant negative impact on the accuracy of different image analysis tasks, as well as prostate tumor localization, thus leading to increased inter- and intra-observer variability. Retrospective bias correction approaches are introduced as a more efficient way of bias correction compared to the prospective methods such that they correct for both of the scanner and anatomy-related bias fields in MR imaging. Previously proposed retrospective bias field correction methods suffer from undesired noise amplification that can reduce the quality of bias-corrected DW-MR image. Here, we propose a unified data reconstruction approach that enables joint compensation of bias field as well as data noise in DW-MR imaging. The proposed noise-compensated, bias-corrected (NCBC) data reconstruction method takes advantage of a novel stochastically fully connected joint conditional random field (SFC-JCRF) model to mitigate the effects of data noise and bias field in the reconstructed MR data. The proposed NCBC reconstruction method was tested on synthetic DW-MR data, physical DW-phantom as well as real DW-MR data all acquired using endorectal MR coil. Both qualitative and quantitative analysis illustrated that the proposed NCBC method can achieve improved image quality when compared to other tested bias correction methods. As such, the proposed NCBC method may have potential as a useful retrospective approach for improving the consistency of image interpretations.

==> future.tex <==
\section{Future Work}
\label{future}
For future work, we will investigate the effect of the proposed bias correction method (NCBC) on the detection accuracies of radiomics-based CAD algorithms previously proposed for prostate cancer detection~\cite{FKhalvati2015,Khalvati2014,KhalvatiMAPS,Khalvati2015_2,Khalvati2015_4,KhalvatiSuperpixel}. These algorithms heavily rely on the quality and intensity homogeneity of regions of interests in similar cases in DW-MRI and therefore, it is expected that compensating for intensity inhomogeneities caused by EMRC will improve the performance. Moreover, the proposed NCBC method will be integrated into CD-MRI algorithms~\cite{CDI,Khalvati2015_1} to investigate whether NCBC improves the separability of cancerous and healthy tissues in prostate for these computationally generated MR sequences. Finally, the $b$-value images of DW-MRI are usually distorted due to patient movement during the image acquisition which may reduce cancer separability. We have presented preliminary results for co-registering the $b$-value images to compensate for patient movement~\cite{Khalvati2015_3}. As future work, we will incorporate the proposed NCBC method with this co-registration algorithm to investigate the effect on the separability of cancerous and healthy tissue in prostate. 
